Experimental study of fish-like bodies with passive tail and tunable stiffness

Scombrid fishes and tuna are efficient swimmers capable of maximizing performance to escape predators and save energy during long journeys. A key aspect in achieving these goals is the flexibility of the tail, which the fish optimizes during swimming. Though, the robotic counterparts, although highly efficient, have partially investigated the importance of flexibility. We have designed and tested a fish-like robotic platform (of 30 cm in length) to quantify performance with a tail made flexible through a torsional spring placed at the peduncle. Body kinematics, forces, and power have been measured and compared with real fish. The platform can vary its frequency between 1 and 3 Hz, reaching self-propulsion conditions with speed over 1 BL/s and Strouhal number in the optimal range. We show that changing the frequency of the robot can influence the thrust and power achieved by the fish-like robot. Furthermore, by using appropriately tuned stiffness, the robot deforms in accordance with the travelling wave mechanism, which has been revealed to be the actual motion of real fish. These findings demonstrate the potential of tuning the stiffness in fish swimming and offer a basis for investigating fish-like flexibility in bio-inspired underwater vehicles.

==> Settings.tex <==





\usepackage[T1]{fontenc}		% Codifica dei font; T1 codifica di output dell'italiano e di lingue occidentali
\usepackage[utf8]{inputenc}		% Codifica degli input; abilita l'utilizzo di caratteri accentati
\usepackage[english]{babel}		% Set the languages; the last one is the main language
\usepackage{geometry}			% Allow to change the margin
\usepackage{setspace}			% Allow to change the interline with \begin{onehalfspaceng} ecc.
\usepackage{fancyhdr}			% Fancy style for page layout
\usepackage{afterpage} 			% Allow to load blank pages with the command '\afterpage{\null\thispagestyle{empty}\clearpage}' 
\usepackage{hyperref}			% Crea collegamenti ipertestuali rendendo cliccabili i riferimenti
\usepackage{url}
\usepackage{color}			% Allow to use colors
\usepackage{xcolor}			% manage colors
\usepackage{enumerate}			% Numbered lists
\usepackage{enumitem}			% Allow to manage the style of the list
\usepackage{graphicx}			% Images
\usepackage{epstopdf}			% allows to convert eps images to pdf for use with pdflatex
\usepackage{pstool}			% Allows to use psfrag with pdflatex (no latex compiler needed)
\usepackage{psfrag}
%\usepackage[normal]{subfigure}		% manage subfigures
\usepackage{subcaption}
\usepackage{subfig}		% manage subfigures
\usepackage{array}			% Tables
\usepackage{tabularx}			% allow to set the width of the whole table
\usepackage[bottom]{footmisc}		% To attach footnote at the end of the page
\usepackage{booktabs}			% is a must for professional-looking layout
\usepackage{longtable}			% is very popular for multi-page tables
\usepackage{caption}			% Captions
\usepackage{float}			% Manage float objects (image, table, ecc.)
\usepackage{subfloat}			% permette la sub numerazione degli oggetti mobili (immagini, tabelle, ecc.)
\usepackage{rotating}			% permette di ruotare immagini, tabelle, ecc. di 90° o di 270°
\usepackage{rotfloat}			% costruisce un ponte tra i pacchetti float e rotating
\usepackage{amsmath} 			% Equations
\usepackage{amssymb}			% Mathematical Symbols
\usepackage{cancel}                     % Simplification Cancellation
\usepackage{mleftright}
\usepackage{listings}                   % Codes
%\usepackage{vector}  			% Allows "\bvec{}" and "\buvec{}" for "blackboard" style bold vectors in maths
\usepackage[swapnames,norules,nouppercase]{frontespizio}
\usepackage[intoc]{nomencl}
\usepackage[acronym,toc,nomain,nopostdot,nonumberlist]{glossaries}
\usepackage[square, numbers, comma, sort&compress]{natbib}
\usepackage{verbatim}                   % Needed for the "comment" environment to make LaTeX comments
\usepackage{wrapfig}                 % Per inserire le figure contornate da testo
\usepackage{blindtext}
\geometry{a4paper,top=2.5cm,bottom=2.5cm,left=2cm,right=2cm,heightrounded,bindingoffset=5mm}
% -------------------------------------- Line-spacing --------------------------------------- %
\linespread{1.2} 
%\linespread{1.5} 
%\linespread{2} 
%\raggedbottom % disattiva lo 'stiracchiamento' del testo; va a favore di spazio bianco a fondo pagina
% ---------------------------------------- Numeration --------------------------------------- %
%\setcounter{secnumdepth}{3} % set the enumeration of the sections
%\setcounter{tocdepth}{3}    % set the enumeration of the sections in the table of contents
%--------------------------------------- Page layout -----------------------------------------%
%\pagestyle{fancy}                       % definisce lo stile di pagina aprendo la strada al pacchetto fancyhdr
%\renewcommand{\chaptermark}[1]{\markright{\chaptername\ \thechapter.\ #1}{}}    % ridefinisce la macro \rightmark per i capitoli
%\renewcommand{\sectionmark}[1]{\markright{\sectionname\ \thesection.\ #1}}      % ridefinisce la macro \rightmark per le sezioni
%\renewcommand{\sectionmark}[1]{\markright{\thesection.\ #1}}
%\lhead{Giacomo Della Posta}             % in alto a sinistra
%\chead{}                                % in alto al centro
%\rhead{\slshape \rightmark}             % in alto a destra (\rightmark contiene ...)
%\lfoot{Giacomo Della Posta}             % in basso a sinistra
%\cfoot{\thepage}                        % in basso al centro (\thepage per mettere il numero di pagina)
%\rfoot{}                                % in basso a destra
%\renewcommand{\headrulewidth}{0.4pt}    % spessore della linea di separazione in alto (0 per eliminare la linea)
%\renewcommand{\footrulewidth}{0.4pt}    % spessore della linea di separazione in basso (0 per eliminare la linea)
\fancypagestyle{plain}{%                                        % modifica dello stile predefinito plain
                        \fancyhf{}                              % cancella tutti i campi di  intestazione e pie di pagina
                        \fancyfoot[R]{\thepage}                 % mette al centro il numero di pagina
                        \renewcommand{\headrulewidth}{0pt}      % spessore della linea di separazione in alto (0 per eliminare la linea)
                        \renewcommand{\footrulewidth}{0.4pt}    % spessore della linea di separazione in basso (0 per eliminare la linea)
                        }                                       % modifica dello stile predefinito plain
\captionsetup{font=small,labelfont=bf,textfont=normalfont,tableposition=bottom,figureposition=bottom}
%\captionsetup{font=small,labelfont=bf,textfont=bf,tableposition=bottom,figureposition=bottom}
% ---------------------------------------- Itemize ------------------------------------------ %
%\setlist[itemize]{noitemsep, topsep=0pt} %Se non vuoi i pallini degli elenchi vuoti, allora commenta queste linee                                     
%\renewcommand{\labelitemi}{$\circ$}	% items i with empty bullets
%\renewcommand{\labelitemii}{$\bullet$}	% items ii with black bullets
\hypersetup{colorlinks=true, linkcolor=black, citecolor=black, filecolor=black, urlcolor=black}
\definecolor{sapienza}{RGB}{130,36,51} % example \definecolor{name}{model}{color-spec}
\definecolor{cust1}{RGB}{85,85,85}
\definecolor{cust2}{RGB}{212,212,212}
\makenomenclature % Generate the nomenclature
\makeglossaries % Generate the glossary
%\lstset{language=[90]Fortran,
%        inputpath=/home/luca/PhD/Thesis/Code,
%        basicstyle=\small\ttfamily, 
%        xleftmargin=0cm,
%        fontadjust=true,
%        keepspaces=true,
%        basewidth=0.5em,
%        breakatwhitespace=false,           % sets if automatic breaks should only happen at whitespace
%        breaklines=false,                  % sets automatic line breaking
%        captionpos=b,                     % b=bottom
%        backgroundcolor=\color{white},
%        identifierstyle=\color{black},
\bibliographystyle{abbrv} % abbrv --> [1], [2], ecc.
%\bibliographystyle{unsrtnat} 

% DEDICATION
%
% The dedication environment makes sure the dedication gets its
% own page and is set out in verse format.

\newenvironment{dedication}
{
  \phantom{.}
  \vspace{13cm}
  \begin{quote} \begin{flushright}}
{\end{flushright} \end{quote}}
\usepackage{calligra}
